Abstraction Refinement Algorithms for Timed Automata

We present abstraction-refinement algorithms for model checking safety properties of timed automata. The abstraction domain we consider abstracts away zones by restricting the set of clock constraints that can be used to define them, while the refinement procedure computes the set of constraints that must be taken into consideration in the abstraction so as to exclude a given spurious counterexample. We implement this idea in two ways: an enumerative algorithm where a lazy abstraction approach is adopted, meaning that possibly different abstract domains are assigned to each exploration node; and a symbolic algorithm where the abstract transition system is encoded with Boolean formulas.

==> app-enum.tex <==
\section{Proofs of Section~\ref{sec-enum}}


\input{algo-refine}

\lemmainclusion*

\begin{proof}
\Refine may only add values to the domain of a
node, so that the refined zone is included in the previous one.
%
%If we did not add any value to the domain, then it means that his parent has
%been modififed.
If~no values were added to the domain of a node, then its parent must
have been modified.  Since $A\subseteq B \Rightarrow
\postta_e(A)\subseteq \postta_e(B)$, the result follows
by induction.
\end{proof}



\lemmacomplete*

\begin{proof}
  We~prove that procedure \Refine preserves
  property~\eqref{Prop1}. Combined with Lemma~\ref{lemma-absr}, this
  entails the result.
  %
  %Since \AbsReach preserves this property, we have to show that \textsf{Refine} preserves it too.
  %\Refine does not add new nodes. It might deletes some nodes.
  First notice that \Refine may not add new nodes. 
  %
  %If we note $n'$ a node $n$ its parent by an edge $e$. After a call to \textsf{Refine}, we have three possibilities:
  Let~$n'$ be a node, $n$ its parent, and $e$ the edge from~$n$ to~$n'$.
  Three cases may arise:
  \begin{itemize}
    \item $n'$ has been modified: then it must have been modified
    at line \ref{refine:modif1} or \ref{refine:modif2}. At this point $n$ is no longer modified, and \Refine ensures that $ \Concrete(n)\subseteq n'.Z$, and  $\Concrete(n)=\postta_{e}(n.Z)$. If
    $n'$ is in \passed, we also have
    $\alpha_{n'.\Dom}(\postta_{e}(n.Z))= n'.Z$.
  \item $n'$ has been deleted: in~this case, if $n$ is part of the subtree and it has either been deleted or moved to \wait, and is not in \passed anymore. Otherwise $n$ is not part of the subtree that has been cut and $n'$ is the root of this subtree, with $n'.Z=\emptyset$ and since $ \Concrete(n)\subseteq n'.Z$.  

  \item $n'$ has not been modified, but $n$~has: then
    using Lemma~\ref{lemma:inclusion}, we~know that the inclusion
    $\postta_{e}(n.Z)\subseteq n'.Z$ (or
    $\alpha_{n'.\Dom}(\postta_{e}(n.Z))\subseteq n'.Z$) is preserved
    by \textsf{Refine}.\qed
\end{itemize}
%So \textsf{Refine} preserves property \ref{prop:Post}.
\let\qed\relax
\end{proof}



\thmalgoenum*


\begin{proof}
We~first prove correctness, assuming termination.  First let us notice
that if the \wait set is empty, then for any reachable location~$l$,
there is a node $n$ such that $n.\ell = l$. This is because
we over-approximate the zones as shown in Lemma~\ref{lemma:complete},
so we over-approximate the set of reachable states.
%
%Knowing this, we can say that
Thus, if $\AbsReach(\TA$, \wait, \passed, $\ell_T)$ returns
$\emptyset$, then $\ell_T$ is not reachable in~$\TA$. In~other words,
if the enumerative algorithm returns "\emph{Not reachable}" then
$\ell_T$ is indeed not reachable.

On the other hand, if the algorithm returns "\emph{Reachable}", it
means that there is a feasible trace reaching~$\ell_T$, and
$\ell_T$~is indeed reachable.

\medskip

%We prove termination for the \textsf{high}\todo{define!} heuristics.
%
Since there are a finite number of possible locations and we can limit
the number of possible zones to a finite number using abstraction
functions, we can deduce that \AbsReach terminates.

Let us assume that the enumerative algorithm does not terminate. Then
it means that \Refine is called infinitely many timed. Note that
\Refine is modifying a node and a node can be modified a
finite number of~time.

We can also note that a node can be destroyed only if one of its
ancestors is modified. As~such, we~can show that for every depth~$k$,
there is a point in the algorithm where every node at depth~$k$ or
less is fixed and will no longer be modified.

So we know that the algorithm does not terminate if, and only~if,
the depth of the
resulting tree is unbounded. This means that there exists a path where
we have two distinct nodes $n_1$ and~$n_2$ with $n_1.\ell = n_2.\ell$
and $n_1.Z = n_2.Z$, since the number of location and possible zones is
finite. Without loss of generality, we can assume that $n_1$ is an ancestor of
$n_2$ and $n_2$ is the parent of another node. This is only possible if
$n_2$ is in \passed, which means that $n_2$ was in \wait and was
not covered at some point. Since a zone can only be modified to be
smaller, this means that $n_2$ has been modified at some
point. Otherwise $n_2$ has always been covered by~$n_1$, which is not
possible. Since $n_2$ has been modified, and it is covered (at~least
by~$n_1$), this means that \cut has been called on~$n_2$ last
time its zone has been modified. This means that $n_2$ has no children
and is not in \passed, contradicting our assumption.
Hence the algorithm always terminates.
\end{proof}


==> app-interp.tex <==
\section{Proof of Section~\ref{section:definitions}}

%\lemmanosimpleinterp*
\begin{restatable}{lemma}{lemmanosimpleinterp}
There exist pairs of zones accepting no simple interpolant.
  %\todo{will move to appendix}
\end{restatable}


\begin{proof}
  Consider 3-dimensional zones $A$, defined as $z=0\et x=y$, and $B$,
  defined as $y\geq 2 \et z\leq 2 \et y-x\leq 1 \et x-z\leq 1$. Both
  zones and their canonical DBMs are represented on
  Fig.~\ref{fig-nosimpleinterp}.
  \begin{figure}[h]
    \centering\noindent
    \begin{minipage}{.45\linewidth}
    \begin{tikzpicture}[scale=1.8,x={(0.45 cm,-0.05 cm)},z={(-0.3 cm,-0.15 cm)},y={(0,0.5 cm)}]
      \draw[-latex'] (0,0,0) -- (3,0,0) node[right] {$x$};
      \draw[-latex'] (0,0,0) -- (0,2.5,0) node[above] {$z$};
      \draw[-latex'] (0,0,0) -- (0,0,4) node[left] {$y$};
      \draw[line width=2pt,black!40!white] (0,0,0) -- (3.5,0,3.5) node[right,black] {$A$}; 
      \fill[black!30!white,draw=black!50!white,line width=2pt,opacity=.4] (1,0,2) -- (1,2,2) -- (3,2,2) -- cycle;
      \fill[black!30!white,draw=black!50!white,line width=2pt,opacity=.4] (1,0,2) -- (3,2,4) -- (3,2,2) node[above right,black,opacity=1] {$B$} -- cycle;
      \fill[black!30!white,draw=black!50!white,line width=2pt,opacity=.4] (1,0,2) -- (1,2,2) -- (3,2,4) -- cycle;
      \fill[black!30!white,draw=black!50!white,line width=2pt,opacity=.4] (1,2,2) -- (3,2,2) -- (3,2,4) -- cycle;
      \begin{scope}
        \draw[dashed] (1,0,2) -- (3,0,2) -- (3,0,4) -- cycle;
        \draw[dotted] (3,2,4) -- (3,0,4);
        \draw[dotted] (3,2,2) -- (3,0,2);
        %
        \draw[dashed] (1,0,0) -- (3,2,0) -- (1,2,0) -- cycle;
        \draw[dotted] (1,0,2) -- (1,0,0);
        \draw[dotted] (3,2,2) -- (3,2,0);
        \draw[dotted] (1,2,2) -- (1,2,0);
        %
        \draw[dashed] (0,0,2) -- (0,2,4) -- (0,2,2) -- cycle;
        \draw[dotted] (1,0,2) -- (0,0,2);
        \draw[dotted] (3,2,4) -- (0,2,4);
        \draw[dotted] (1,2,2) -- (0,2,2);
      \end{scope}
    \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{.5\linewidth}
      \newcolumntype{C}{>{\centering $(}p{13mm}<{)$}}
      \[
      A = \left(\begin{array}{CCCC}
        0,\le & +\infty,< & +\infty,< & 0,\le \tabularnewline
        +\infty,< & 0,\le & 0,\le & +\infty,< \tabularnewline
        +\infty,< & 0,\le & 0,\le & +\infty,< \tabularnewline
        0,\le & +\infty,< & +\infty,< & 0,\le 
      \end{array}\right)
      \]
      \newcolumntype{C}{>{\centering $(}p{13mm}<{,\le)$}}
      \[
      B = \left(\begin{array}{CCCC}
        0 & 3 & 4 & 2 \tabularnewline
        -1 & 0 & 1 & 1 \tabularnewline
        -2 & 1 & 0 & 0 \tabularnewline
        0 & 1 & 2 & 0 
      \end{array}\right)
      \]
    \end{minipage}
    \caption{Two zones that cannot be separated by a simple interpolant}
    \label{fig-nosimpleinterp}
  \end{figure}

  We~observe that they are disjoint: if a triple~$(x,y,z)$ were in
  both~$A$ and~$B$, then $x=y$ and~$z=0$ (for being in~$B$); in~$A$,
  $y\geq2$, hence also $x\geq 2$, contradicting $x-z\leq 1$.

  Now, assume that there is a simple interpolant~$I$, with~$A\cap
  I=\emptyset$ and $B\subseteq I$. In~the canonical DBM of~$I$, only
  one non-diagonal element is not~$(+\infty,<)$; assume
  $I(x,y)\not=(+\infty,<)$. Then we~must have
  $A(y,x)+I(x,y) < (0,\mathord\leq)$,
  and
  $B(x,y)\leq I(x,y)$. Then $A(x,y)+B(x,y) < (0,\mathord\leq)$. However, it~can
  be observed that in our example, $A(x,y)+B(y,x)\geq (0,\mathord\leq)$ for all
  pairs~$(x,y)$.
\end{proof}



\lemmasmallinterp*

\begin{proof}
  Assume that $A$ and~$B$ are given as canonical DBMs, which we also
  write~$A$ and~$B$ for the sake of readability.  We prove the
  stronger result that $A\cap B=\emptyset$ if, and only~if, for
  some~$n\leq \size{\Clocksz}/2$, there exists a sequence of
  pairwise-distinct clocks $(x_i)_{0\leq i\leq 2n-1}$ such that,
  writing~$x_{2n}=x_0$, 
  \[
  \sum_{i=0}^{n-1} A(x_{2i},x_{2i+1}) + B(x_{2i+1},x_{2i+2}) < (0,\leq).
  \]
  Before proving this result, we~explain how we conclude the proof:
  the inequality above entails that
  \[
  \bigcap_{i=0}^{n-1} A(x_{2i},x_{2i+1})
  \cap
  \bigcap_{i=0}^{n-1} B(x_{2i+1},x_{2i+2}) = \emptyset
  \]
  where we abusively identify $A(x,y)$ with the half-space it
  represents.  It~follows that $\bigcap_{i=0}^{n-1}
  B(x_{2i+1},x_{2i+2})$ is an interpolant, whose density is less than
  or equal to~$\size\Clocksz/2$.
  
  Assume that such a sequence exists, and write~$C$ for the
  DBM $\min(A, B)$. Then
  \begin{xalignat*}1
    \sum_{i=0}^{2n-1} C(x_{i},x_{i+1}) &=
    \sum_{i=0}^{2n-1} \min \{A(x_{i},x_{i+1}),B(x_{i},x_{i+1})\}
    \\ &
    \le \sum_{i=0}^{n-1} A(x_{2i},x_{2i+1}) + B(x_{2i+1},x_{2i+2})
      < (0,\leq).
  \end{xalignat*}
  This entails that the intersection is empty.

  Conversely, if the intersection is empty, then there is a sequence
  of clocks $(x_i)_{0\leq i<m}$, with~$m\leq\size\Clocksz$, such that,
  letting $x_m=x_0$, we~have
  \[
  \sum_{i=0}^{m-1} \min\{A(x_i,x_{i+1}), B(x_i,x_{i+1})\} < (0,\leq).
  \]
  Consider one of the shortest such sequences.  Since~$A$ and~$B$ are
  non-empty, the sum must involve at least one element of each
  DBM. Moreover, if~it involves two consecutive elements of the same
  DBM (i.e., if $A(x_i,x_{i+1}) < B(x_i,x_{i+1})$ and
  $A(x_{i+1},x_{i+2}) < B(x_{i+1},x_{i+2})$ for some~$i$), then by
  canonicity of the DBMs of~$A$ and~$B$, we~can drop clock~$x_{i+1}$
  from the sequence and get a shorter sequence satisfying the same
  inequality, contradicting minimality of our sequence. The~result follows.
\end{proof}



\propniminterp*

\begin{proof}
%  
  \begin{figure}[t]
    \begin{algorithm}[H]
      \small
      \KwInput{canonical DBM $A$, $B$}\;
      \For{$(x,y)\in \Clocksz^2$}{%
        \eIf{$A(x,y)\leq B(x,y)$}
           {$M^0(x,y):=A(x,y)$\;}
           {$M^0(x,y):=(\infty,<)$\;}
      }
      $N^0:=\canonical(M^0)$\;
      \For{($i=1$; $i\leq \size\Clocksz/2$; $i++$)}
          {
            \For {$(x,y)\in \Clocksz^2$}
                 {
                   $M^i(x,y):= \min\{N^{i-1}(x,y),
                      \min_{z\in\SC_B(y)} N^{i-1}(x,z)+B(z,y)\}$\;
                 }
            \For {$(x,y)\in \Clocksz^2$}
                 {
                   $N^i(x,y):= \min\{M^{i}(x,y),
                      \min_{z\in\SC_A(y)} M^{i}(x,z)+A(z,y)\}$\;
                   \If{$(x=y)$ and $N^i(x,x)<(0,\mathord\leq)$}
                      {\Return ($\texttt{true}, i$)\;}
                 }
          }
          \Return \texttt{false}\;
      \caption{Algorithm for minimal interpolant}
      \label{alg:interpol}
      \label{alg-interpol}
    \end{algorithm}
\end{figure}

Algorithm~\ref{alg-interpol} describes our procedure. In~order to prove
its correctness, we~begin with proving that the sequence of DBM it computes
satisfies the following property:
\begin{lemma}
%For any~$0\leq i\leq \size\Clocksz/2$ and
  For any~$i\geq 0$ such that $N^i$ has been computed by
  Algorithm~\ref{alg:interpol}, for any $(x,y)\in\Clocksz^2$, it~holds
  \[
  N^i(x,y) = \min_{\substack{\pi\in\Paths(x,y)\\\size\pi_B\leq i}} W_{\min(A,B)}(\pi).
  \]
\end{lemma}

\begin{proof}
The proof proceeds by induction on~$i$.  For~$i=0$, pick a
path~$\pi=(x_i)_{0\leq i\leq k}$ from~$x+0$ to~$x_k$ such that
$\size\pi_B=0$. Then
\begin{xalignat*}1
  W_{\min(A,B)}(\pi) &= \sum_{0\leq i<k} A(x_i,x_{i+1}) 
  %\\ &
  = \sum_{0\leq i<k} M^0(x_i,x_{i+1}) \\
   &= \sum_{0\leq i<k} N^0(x_i,x_{i+1}) \geq N^0(x_0,x_k).
\end{xalignat*}
The first two equalities follow from the fact that $\pi$ only involves
transitions in~$E_{A\leq B}$; the third equality is because
canonization will not modify entries from~$A$ (since $A$ is originally
in canonical form). The~last inequality follows from canonicity of~$N^0$.

Now assume that the result holds at step~$i$, and that $N^{i+1}$ is
defined. Pick~$x$ and~$y$ in~$\Clocksz$. By~construction of~$M^{i+1}$
and~$N^{i+!}$, there exists $z$ and~$t$ in~$\Clocksz$ such that
$N^{i+1}(x,y) = N^i(x,z)+B(z,t)+A(t,y)$ with $t\in \SC_A(y)$
(or~$t=y$) and $z\in\SC_B(t)$ (or~$z=t$).  From the induction
hypothesis, there is a path~$\pi'$ from~$x$ to~$z$ such that
$N^i(x,z)=W_{\min(A,B)}(\pi')$, and~$\size{\pi'}_B\leq i$. Adding~$t$
and~$y$ to this path, we~get a path~$\pi$ from~$x$ to~$y$ such that
$N^{i+1}(x,y) = W_{\min(A, B)}(\pi)$ and $\size\pi_B\leq i+1$.

It~remains to prove that any path~$\pi$ from~$x$ to~$y$ with
$\size\pi_B\leq i+1$ is such that $N^{i+1}(x,y) \leq W_{\min(A,
  B)}(\pi)$. Fix such a path $\pi=(x_j)_{0\leq j\leq k}$\;
we~concentrate on the case where $\size\pi_B=i+1$, since the other
case follows from the induction hypothesis. We~decompose~$\pi$
as~$\pi_1=(x_j)_{0\leq j\leq l}$, $\pi_2=(x_l,x_{l+1})$ and
$\pi_3=(x_j)_{l+1\leq j\leq k}$, such that $(x_l,x_{l+1})\in E_B$ and
$(x_j,x_{j+1})\in E_A$ for all~$j>l$; in~other terms, $\pi_2$ is the
last $E_B$ transition of~$\pi$, and $\pi_3$~is a path from~$x_{l+1}$
to~$x_k$ only involving transitions in~$A$. Then
\[
w_{\min(A, B)}(\pi_2\cdot\pi_3) = B(x_l,x_{l+1}) + w_A(\pi_3)
\geq  B(x_l,x_{l+1}) + w_{A}(x_{l+1},x_k),
\]
and
\begin{itemize}
\item if $(x_{l+1},x_k)\in E_B$, then $w_{\min(A,B)}(\pi_2\cdot\pi_3)
  \geq w_B(x_l,x_k)$, and, applying the induction hypothesis, 
  $w_{\min(A, B)}(\pi) \geq N^i(x,x_l)+\min\{A(x_l,x_k), B(x_l,x_k)\}$.
  Since $M^{i+1}(x,x_l)\leq N^i(x,x_l)$, we~get
  \begin{xalignat*}1
  w_{\min(A, B)}(\pi) &\geq \min\{N^i(x,x_l)+B(x_l,x_k), M^{i+1}(x,x_l)+A(x_l,x_k)\}
  \\ &\geq N^{i+1}(x,x_k).
  \end{xalignat*}
\item if $(x_{l+1},x_k)\in E_B$, then $w_{\min(A,B)}(\pi_2\cdot \pi_3)
  \geq B(x_l,x_{l+1}) + A(x_{l+1}, x_k)$. From the induction
  hypothesis, $w_{\min(A, B)}(\pi) \geq N^i(x,x_l)+B(x_l,x_{l+1}) +
  A(x_{l+1},x_k) \geq N^{i+1}(x,x_k)$.\qed
\end{itemize}
\let\qed\relax
\end{proof}

Following the argument of the proof of Lemma~\ref{lemma-smallinterpol}, we~get:
\begin{corollary}
If $A \cap B\not=\emptyset$, then Algorithm~\ref{alg:interpol} returns
\texttt{\textup{false}}; otherwise, it~returns
$(\texttt{\textup{true}},k)$ for the smallest~$k$ such that for all
cyclic path~$\pi$ such that $\size\pi_B<k$, it~holds $w_{\min(A, B)}(\pi)\geq (0,\leq)$.
\end{corollary}
This entails that $k$ is the dimension of the minimal interpolant. The
minimal interpolant can be obtained by taking the $B$-elements of the
negative cycle found by the algorithm.
\end{proof}


==> app-symb.tex <==
\section{Proofs of Section~\ref{sec-symb}}

\subsection{Reduction}
\label{section:reduction}
We now define the reduction operation, which is similar to the
reduction of DBMs.  The~idea is to eliminate unsatisfiable minterms
from a given Boolean formula.  For~example, we~would like to make sure
that in all minterms, if~$p_{x-y\leq 1}$ holds, then so
does~$p_{x-y\leq 2}$, when both are available predicates.  Another
issue is to eliminate minterms that are unsatisfiable due to triangle
inequality.  This is similar to the shortest path computation used to
turn DBMs in canonical form.

Let a \emph{path} in~$\Dom$ be a sequence
$x_1,(\alpha_1,\mathord{\prec_1}),x_2,(\alpha_2,\mathord{\prec_2}), \ldots,
x_k,(\alpha_k,\mathord{\prec_k}),x_{k+1}$ where~$x_1,\ldots,x_{k+1} \in
\Clocksz$, and~$(\alpha_i,\mathord{\prec_i}) \in \Dom_{x_i,x_{i+1}}$ for $1\leq
i\leq k$.  Let us define $\Paths_k^\Dom(x-y\prec \alpha)$ as the set
of paths from~$x$ to~$y$ of length~$k$ and weight at
most~$(\alpha,\mathord\prec)$, that~is,
paths~$x_1,(\alpha_1,\mathord{\prec_1}),x_2,(\alpha_2,\mathord{\prec_2}), \ldots,
x_k,(\alpha_k,\mathord{\prec_k}),x_{k+1}$ with~$x_1=x$, $x_{k+1} = y$,
and~$\sum_{i=1}^k (\alpha_i,\mathord{\prec_i}) \leq (\alpha,\mathord\prec)$.
We~also
denote~${\Paths_{\leq k}^\Dom(x-y\prec \alpha)} = \bigcup_{l\leq k}
\Paths_l^\Dom(x-y\prec \alpha)$.  For a
path~$\pi=x_1,(\alpha_1,\mathord{\prec_1}),\ldots,x_{k+1}$ and minterm~$v$, let
us write~$v \models \pi$ for the statement $v \models \wedge_{i=1}^k
\clpred{x_i - x_{i+1}\prec \alpha_i}$.

A~minterm~$v \in \bbB^{\Pred}$ is \emph{$k$-reduced} if for all 
$(x,y) \in \Clocksz^2$ and~$(\alpha,\mathord\prec) \in \Dom_{x,y}$, 
for all~$\pi = x_1,{(\alpha_1,\mathord{\prec_1})},x_2, \ldots,x_{k+1} \in \Paths_{\leq k}(x-y\prec \alpha)$,
%$x_1,\ldots,x_k,x_{k+1} \in \Clocksz$ and~$(\alpha_i, \mathord{\prec_i})\in \Dom_{x_i,x_{i+1}} \times \{<,\leq\}$
%for~$1\leq i\leq k$,
%whenever~$v \models \wedge_{i=1}^k p_{x_i-x_{i+1} \prec_i \alpha_i}$, 
whenever $v \models \pi$, we also have $v \models \clpred{x_1 -
  x_{k+1}\prec \alpha}$ for all~$(\alpha,\mathord\prec) \in
\Dom_{x_1,x_{k+1}}$ with $(\alpha,\mathord\prec) \geq \sum_{i=1}^k
(\alpha_i,\mathord{\prec_i})$.
% \[
% v \models \bigwedge_{\substack{(\alpha,\mathord\prec) \in \Dom_{x_1,x_{k+1}} :\\(\alpha,\mathord\prec) \geq \sum_{i=1}^k (\alpha_i, \mathord\prec_i)}} p_{x_1-x_{k+1} \prec \alpha}.
% \]
%then for all~$(\alpha,\mathord\prec) \in \Dom_{x_1,x_{k+1}}$ with $(\alpha,\mathord\prec) \geq \sum_{i=1}^k (\alpha_i, \mathord\prec_i)$,
%we have $v \models p_{x_1-x_{k+1} \prec \alpha}$.
Thus, in a~$k$-reduced minterm, no~contradictions can be obtained via
paths of length less than or equal to~$k$.  Observe that
$|\Clocksz|$-reduction is equivalent to satisfiability since the
condition then includes all paths, and it is known that in the absence
of negative cycles, a~set of difference constraints is
satisfiable. Furthermore, for the concrete domain, $k$-reduction is
equivalent to reduction for any~$k\geq 2$.  A formula is said to be
$k$-reduced if all its minterms are $k$-reduced.

\begin{example}
  \label{example:reduced}
  Given predicates $\Pred = \{\clpred{x-y\leq 1}, \clpred{y-z\leq 1},
  \clpred{x-z\leq 2}\}$, the formula $\clpred{x-y\leq 1} \land
  \clpred{y-z\leq 1}$ is not reduced since it contains the
  unsatisfiable minterm $\clpred{x-y\leq 1} \land \clpred{y-z\leq 1}
  \land \lnot \clpred{x-z\leq 2}$.  However, the same formula is
  reduced if~$\Pred = \{\clpred{x-y\leq 1}, \clpred{y-z\leq 1}\}$.

  Consider now the predicate set~$\calP = \{\clpred{x-y\leq 1},
  \clpred{y-z\leq 1}, \clpred{z-w\leq 3}, \clpred{x-w\leq 5}\}$, and
  consider the formula~$\phi = \clpred{x-y\leq 1}\land \clpred{y-z\leq
    1} \land \clpred{z-w\leq 3}$ which is~$2$-reduced.  Notice that
  the reduction of~$\phi$ is $\clpred{x-y\leq 1}\land \clpred{y-z\leq
    1} \land \clpred{z-w\leq 3} \land \clpred{x-w\leq 5}$ since the
  last predicate is implied by the conjunction of others.  However,
  $\phi$ is $2$-reduced since no path of length~$2$ allows to
  deduce~$\clpred{x-w \leq 5}$.  In~the concrete domain,
  $\clpred{x-y\leq 1} \land \clpred{y-z \leq 1}$ would imply
  $\clpred{x-z\leq 2}$, thus, $\clpred{x-w\leq 5}$ could be derived~too.
  It~is indeed because of the abstract domain that $2$-reduction
  might fail to capture all shortest paths.
%  Similarly, it is possible to have $2$-reduced minterms which are unsatisfiable.
\end{example}

In this paper, we only consider $2$-reduction since computing
reductions is the most expensive operation in our algorithms, and the
formula below defining $2$-reduction already tends to grow in~size.
Let us define $\reduce_\Dom^2$ as follows
\[
  \bigwedge_{\substack{(x,y) \in \Clocksz^2\\ (k,\mathord{\prec}) \in \Dom_{x,y}}}
  \Biggl[\clpred{x-y \prec k} \leftarrow
  \Bigl(
    \bigvee_{
      \substack{
        (l_1,\mathord{\prec_1}) \in \Dom_{x,y}\\
        (l_1,\mathord{\prec_1}) \leq (k,\mathord{\prec})
      }
    } \clpred{x-y\prec_1 l_1} \lor \!\!\!\!
    \bigvee_{
      \substack{z \in \Clocksz,
        (l_1,\mathord{\prec_1}) \in \Dom_{x,z}, \\
        (l_2,\mathord{\prec_2}) \in \Dom_{z,y}\\
        (l_1,\mathord{\prec_1})+(l_2,\mathord{\prec'_2})\leq (k,\mathord{\prec})
      }
    }
    \!\!\!\!
    \clpred{x-z\prec_1 l_1} \mathrel{\wedge} \clpred{z-y\prec_2 l_2}
  \Bigr)\Biggr]
\]
The formula intuitively applies shortest paths over
paths of length $1$ or~$2$.

%\begin{lemma}
%% \begin{restatable}{lemma}{lemmareduce}
%% \label{lemma:reduce}
%%   % Let~$S$ be any Boolean formula on predicates~$\Pred$,
%%   % and~$k\geq 2$.
%%   For all formulas~$S(\Pred)$,
%%   we have $\sem{S}_\Dom = \sem{\reduce_\Dom^2(S)}_\Dom$
%%   and all minterms of~$\reduce_\Dom^2(S)$ are $2$-reduced.
%% \end{restatable}
%\end{lemma}

\lemmareduce*

%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}%[of Lemma~\ref{lemma:reduce}]
  It is easy to see that $\sem{\reduce_\Dom^k(S)}_\Dom \subseteq \sem{S}_\Dom$.
  In fact, any minterm of the former is a minterm of~$S$ as well by definition.

  To see the converse, consider~$v \in \minterms(S)$. We show
  that~$\sem{v}_\Dom \subseteq \sem{\reduce_\Dom^k(S)}_\Dom$.
  If~$\sem{v}_\Dom = \emptyset$ then the inclusion holds trivially.
  Otherwise, we must have $v \in \minterms(\reduce_\Dom^k(S))$. In
  fact, we show that all minterms~$v \not \in
  \minterms(\reduce_\Dom^k(S))$ satisfy~$\sem{v} = \emptyset$.
  Consider such a minterm~$v$. There must exist~$x,y \in \Clocksz$ and
  $(k,\prec_k) \in \Dom_{x,y}$ such that~$\lnot \clpred{x-y\prec k}$ but
  the right hand side of the implication holds.  But this implies
  that~$\sem{v} = \emptyset$.

  The fact that all miterms of $\reduce_\Dom^k(S)$ are $k$-reduced
  follow by the definition of the operator.
\end{proof}
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{example}
  Note that~$\reduce_\Dom^2(S)$ can still contain valuations that are
  unsatisfiable.  Consider $\Pred=\{ \clpred{x-y\leq 1}, \clpred{y-z\leq 1},
  \clpred{x-z\leq 4}, \clpred{z-x\leq -3}\}$.  Then the minterm~$u$ that sets
  all predicates to true is still contained in $\reduce_\Dom^2(S)$
  although~$\sem{u} = \emptyset$ since~$x-y\leq 1 \land y-z\leq 1$
  implies~$x-z\leq 2$ which contradicts~$z-x\leq -3$.  Here, adding
  the predicate~$\clpred{x-z\leq 2}$ or~$\clpred{x-z<3}$ would render the
  abstraction precise enough to eliminate this valuation
  in~$\reduce_\Dom^2(S)$.
\end{example}

Let us see how an abstraction can be refined so that the reduced constraint
eliminates a given unsatisfiable minterm.
%\begin{lemma}
%% \begin{restatable}{lemma}{lemmaemptyrefine}
%% \label{lemma:empty-refine}
%%   Let~$v \in \bbB^{\Pred^\Dom}$ be a minterm such
%%   that~$v \models \reduce_\Dom^2$ and
%%   $\sem{v} = \emptyset$.
%%   One~can compute in polynomial time a refinement~$\Dom' \supset \Dom$
%%   such that~$v \not \models \reduce_{\Dom'}^2$.
%% \end{restatable}
%\end{lemma}

\lemmaemptyrefine*

%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}%[of Lemma~\ref{lemma:empty-refine}]
  Consider a (non-canonial) DBM~$D$ that encodes~$v$. Formally, for
  all~$(x,y) \in \Clocksz^2$, $D(x,y) = \min \{ (k,\mathord\prec)
  \mid \clpred{x - y \prec k} \in \Pred_{x,y}\text{ and } v(\clpred{x - y \prec
    k}) = 1\}$.  The~corresponding graph must have a negative
  cycle~$s_1s_2\ldots s_m$ with $s_m = s_1$.  To~define~$\Dom'$,
  we~add the following predicates to~$\Dom$:
  \begin{itemize}
    \item $s_i - s_{i+1} \leq D(s_i,s_{i+1})$ for all~$1\leq j \leq m-1$.
    \item $s_1 - s_{j} \leq D(s_1,s_2) + D(s_2,s_3) + \ldots + D(s_{j-1},s_{j})$
      for~$1\leq j\leq m-1$.
    \end{itemize}
    Intuitively, along the negative cycle, we are adding predicates to
    represent exactly each single step, and also each big step from
    $s_1$ to~$s_j$. This allows to derive the negative cycle using
    only paths of length~$2$.

    More precisely, $v \land \reduce^2_{\Dom'}$ implies the following
    two predicates: $s_1 - s_m \leq \sum_{j=1}^{m-1} D(s_j,s_{j+1})$,
    and $s_m - s_1 \leq D(s_m,s_1)$ as implied by~$v$.  Since
    $-D(s_m,s_1) > \sum_{j=1}^{m-1} D(s_j,s_{j+1})$ due to the
    negative cycle, the~first predicate implies $\lnot \clpred{s_1 -
      s_m \leq -D(s_m,s_1)}$, which contradicts the second one. Hence~$v
    \not \models \reduce^2_{\Dom'}$.
\end{proof}
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Successor Computation}
%We represent sets of zones as propositional formulas over
%the predicates~$\Bits\cup\Pred$.
%Recall that we represent a set of extended zones as a formula
%over predicates~$\Bits \cup \Pred$.
In this section, we explain how successor computation is realized in
our encoding.
%
For a guard~$g$, assume we have computed an
abstraction~$\alpha_\Dom(g)$ in the present abstract domain. 
% (see
%Appendix~\ref{section:abs-compute}).
%\todo{fix ref...}
%
For each transition~$\sigma=(\ell_1,g,R,\ell_2)$, let us define the
formula~$T_\sigma = \ell_1 \land \alpha_\Dom(g)$.  We~show how each
basic operation on zones can be computed in our BDD encoding.
In~our algorithm, all formulas~$A(\Bits,\Pred)$ representing sets of
states are assumed to be reduced, that is, $A(\Bits,\Pred) \subseteq
\reduce_\Dom^2(A(\Bits,\Pred))$.

%\paragraph{Intersection}

\medskip
The~intersection operation is simply logical conjunction.
% In fact, given $A(\Bits,\Pred)$ and~$B(\Bits, \Pred)$,
% we define $A(\Bits, \Pred) \sqcap B(\Bits, \Pred) = \reduce(A(\Bits, \Pred) 
% \land B(\Bits, \Pred))$.

%\begin{lemma}
%% \begin{restatable}{lemma}{lemmainter}
%% \label{lemma:inter}
%%   For all reduced formulas~$A(\Pred), B(\Pred)$,
%%   $A(\Pred) \land B(\Pred) = \alpha_\Dom(\sem{A(\Pred)}_\Dom \cap \sem{B(\Pred)}_\Dom)$.
%% \end{restatable}
%\end{lemma}
\lemmainter*

\begin{proof}%[of Lemma~\ref{lemma:inter}]
  Consider~$v \in \minterms(A(\Pred) \land B(\Pred))$.  Then $v \in
  \minterms(A(\Pred)) \cap \minterms(B(\Pred))$.  So~$\sem{v}
  \subseteq \sem{A(\Pred)} \cap \sem{B(\Pred)}$, and~$v =
  \alpha_\Dom(\sem{v}) \subseteq \alpha_\Dom(\sem{A(\Pred)}_\Dom \cap
  \sem{B(\Pred)}_\Dom)$.

  We will now show $\alpha_\Dom(\sem{A(\Pred)}_\Dom \cap
  \sem{B(\Pred)}_\Dom) \subseteq A(\Pred) \land B(\Pred)$, which is
  equivalent to $\sem{A(\Pred)}_\Dom \cap \sem{B(\Pred)}_\Dom
  \subseteq \sem{A(\Pred) \land B(\Pred)}$.  Consider any clock
  valuation~$\nu$ in the LHS, and let~$v = \alpha_\Dom(\nu)$.
  Since~$\nu \in \sem{A(\Pred)}_\Dom$ and~$\nu \in
  \sem{B(\Pred)}_\Dom$, we must have $v \in A(\Pred) \land B(\Pred)$,
  so $\nu \in \sem{A(\Pred) \land B(\Pred)}$.
%  By Lemma~\ref{lemma:reduce}, the latter set is equal to~$\sem{A(\Pred) \land B(\Pred)}$.
\end{proof}


\medskip
%\paragraph{Time Successors}
%Define the following relation.
For the time successors, we define
% \[
% S_{\Up} = 
% \bigwedge_{\substack{x,y \in \Clocksz\\ (k,\prec) \in \Dom_{x,y}}}
%   p_{x-y\prec k}' \leftrightarrow
% 	\left\{
% 	\begin{array}{ll}
% 		\{\texttt{true},\texttt{false}\} & \text{if } y = 0,\\
% 		p_{x-y \prec k} & \text{ otherwise.}
% 	\end{array}
% 	\right.
% \]
% \[
\[
S_{\Up} = 
 \bigwedge_{\substack{x \in \Clocks\\ (k,\prec) \in \Dom_{x,0}}}
 (\lnot \clpred{x-0\prec k} \rightarrow \lnot \clprpr{x-0\prec k})
 \bigwedge_{\substack{x,y \in \Clocksz, x\neq 0\\ (k,\prec) \in \Dom_{x,y}}}
 (\clprpr{x-y\prec k} \leftrightarrow \clpred{x-y \prec k}).
 \]
Note that this relation is not a function: for~$x\leq 0,
y=0$, if~$\lnot \clpred{x-y\prec k}$, then necessarily $\lnot
\clprpr{x-y\prec k}$; but otherwise both truth values for~$\clprpr{x-y\prec
  k}$ are allowed.  In~fact, the~formula only says that all lower
bounds on clocks and diagonal constraints must be preserved.
We~let $\Up(A(\Bits,\Pred)) = \reduce(\postop_{S_\Up}(A(\Bits,\Pred)))$.

\begin{figure}[t]
  \centering
  \begin{tikzpicture}
    \begin{scope}[scale=.45]
      \fill[black!40] (0,0) -- (2,0) -- (2,1) -- (1,1)-- cycle;
      \draw[-latex',line width=.6pt] (0,0) -- (5.5,0);
      \draw[-latex',line width=.6pt] (0,0) -- (0,4.5);
      \node at (0,5) {$y$};
      \node at (6,0) {$x$};
      \begin{scope}[line width=0.1pt]
        \draw[-] (1,0) -- (1,4.5);
        \draw[-] (2,0) -- (2,4.5);
        \draw[-] (3,0) -- (3,4.5);
        \draw[-] (4,0) -- (4,4.5);
        \draw[-] (5,0) -- (5,4.5);
        \draw[-] (0,1) -- (5.5,1);
        \draw[-] (0,2) -- (5.5,2);
        \draw[-] (0,3) -- (5.5,3);
        \draw[-] (0,4) -- (5.5,4);
        \draw[-] (0,0) -- (4.5,4.5);
        \draw[-] (1,0) -- (5.5,4.5);
        \draw[-] (2,0) -- (5.5,3.5);
        \draw[-] (3,0) -- (5.5,2.5);
        \draw[-] (0,1) -- (3.5,4.5);
        \draw[-] (0,2) -- (2.5,4.5);
        \draw[-] (0,3) -- (1.5,4.5);
      \end{scope}
      \begin{scope}[line width=1.5pt,color=red]
        \draw[-] (0,1) -- (5.5,1);
        \draw[-] (2,0) -- (2,4.5);
        \draw[-] (3,0) -- (3,4.5);
        \draw[-] (0,0) -- (4.5,4.5);
        \draw[-] (4,0) -- (5.5,1.5);
      \end{scope}
    \end{scope}
  \end{tikzpicture}
%  ~~~~~~~
\hfil
  \begin{tikzpicture}
    \begin{scope}[scale=.45]
      \draw[-latex',line width=.6pt] (0,0) -- (5.5,0);
      \draw[-latex',line width=.6pt] (0,0) -- (0,4.5);
      \fill[pattern=north west lines, pattern color=blue]
      (0,0) -- (4.5,4.5) -- (5.5,4.5) -- (5.5,1.5) -- (4,0) -- cycle;
      \node at (0,5) {$y$};
      \node at (6,0) {$x$};
      \begin{scope}[line width=0.1pt]
        \draw[-] (1,0) -- (1,4.5);
        \draw[-] (2,0) -- (2,4.5);
        \draw[-] (3,0) -- (3,4.5);
        \draw[-] (4,0) -- (4,4.5);
        \draw[-] (5,0) -- (5,4.5);
        \draw[-] (0,1) -- (5.5,1);
        \draw[-] (0,2) -- (5.5,2);
        \draw[-] (0,3) -- (5.5,3);
        \draw[-] (0,4) -- (5.5,4);
        \draw[-] (0,0) -- (4.5,4.5);
        \draw[-] (1,0) -- (5.5,4.5);
        \draw[-] (2,0) -- (5.5,3.5);
        \draw[-] (3,0) -- (5.5,2.5);
        \draw[-] (0,1) -- (3.5,4.5);
        \draw[-] (0,2) -- (2.5,4.5);
        \draw[-] (0,3) -- (1.5,4.5);
      \end{scope}
      \begin{scope}[line width=1.5pt,color=red]
        \draw[-] (0,1) -- (5.5,1);
        \draw[-] (2,0) -- (2,4.5);
        \draw[-] (3,0) -- (3,4.5);
        \draw[-] (0,0) -- (4.5,4.5);
        \draw[-] (4,0) -- (5.5,1.5);
      \end{scope}
    \end{scope}
  \end{tikzpicture}
  \caption{Time successors: the successors of the gray zone on the left are the
  union of all blue dashed zones on the right.}
  \label{fig:up}
\end{figure}


\begin{example}
Figure~\ref{fig:up} shows this operation applied to the gray zone on the left.
The overapproximation is visible in this example. In~fact,
the blue dashed zone defined by $Z = 3< x< 5 \land 0\leq y< 1 \land x-y< 4$
(on the bottom right) is computed as a successor of the gray zone
although no point of the gray zone can actually reach~$Z$ by a time delay.
Adding more diagonal constraints to the abstract domain, for instance, 
$x-y\leq 2$ would eliminate this successor.
\end{example}

%\begin{lemma}
%% \begin{restatable}{lemma}{lemmaup}
%% \label{lemma:up}
%% 	For any Boolean formula~$A(\Bits, \Pred)$,
%%     $\alpha_\Dom(\timesucc{\sem{A}})\subseteq \Up(A)$.
%%     Moreover, if~$\Dom$ is the concrete domain and $A$ is reduced, 
%%     then this holds with equality.    
%% \end{restatable}
%\end{lemma}
\lemmaup

\begin{proof}%[of Lemma~\ref{lemma:up}]
  We show that 
  $\alpha_\Dom(\timesucc{\sem{A}})\subseteq \Up(A)$,
  which is equivalent to 
  $\timesucc{\sem{A}}\subseteq \sem{\Up(A)}_\Dom$.
  Let~$\nu' \in \timesucc{\sem{A}}$, and let~$\nu \in \sem{A}$ such that
  $\nu' = \nu + d$ for some~$d\geq 0$.
  We write~$u = \alpha_\Dom(\nu)\in \minterms(A)$, and~$v = \alpha_\Dom(\nu')$.
  We now show that~$(u,v) \in S_\Up$. This suffices to prove the inclusion since
  $v \in \minterms(\Up(A))$ implies that~$\nu' \in \sem{v}_\Dom \subseteq \sem{\Up(A)}_\Dom$.
  Observe that $\alpha_\Dom(\nu)$ and~$\alpha_\Dom(\nu')$ satisfy the same diagonal predicates
  of the form~$p_{x-y\prec \alpha}$ with~$x,y \neq 0$, since~$\nu' = \nu+d$.
  Moreover, any lower bound satisfied by~$u$ is also satified by~$v$. Thus, $(u,v) \in S_\Up$.

  \smallskip
  Assume now that~$A$ is reduced. We show that $\Up(A) \subseteq \alpha_\Dom(\timesucc{\sem{A}})$.
  Let~$v \in \minterms(\Up(A))$, and let~$(u,v) \in S_\Up$ with~$u \in \minterms(A)$.
  We claim that~$\sem{v} \subseteq \timesucc{\sem{u}}$.
  This suffices to prove the inclusion since 
  $\{v\} = \alpha_\Dom(\sem{v}) \subseteq \alpha_\Dom(\timesucc{\sem{u}}) \subseteq \alpha_\Dom(\timesucc{\sem{A}})$.
  To~prove the claim, it~suffices to see~$\sem{u}$ and~$\sem{v}$ as DBMs. In fact, $S_\Up$ precisely corresponds to the up operation
  on DBMs. In particular, $u$ and~$v$ have the same diagonal constraints, and any lower bound of~$u$ is a lower bound of~$v$.
  Because~$u$ is reduced, this implies that~$\timesucc{\sem{v}}
  \subseteq \sem{u}$.
\end{proof}


\begin{example}
  Note that we do need that the domain is concrete to prove
  equality. In~fact, assume the predicates are $p_1 = y-x\leq 3$,
  $p_2= x-y\leq 1$, $x\leq 1, y\leq 2, x\leq 2, y\leq 4$.  Then if
  $u=x\leq 1\land y\leq 2\land p_1\land p_2$ and~$v=1\leq x\leq 2\land
  y\leq 4\land p_1\land p_2$.  So~$v$ is larger than $\timesucc{u}$.

  Second, to see that the $\Up$ operation can yield strict
  over-approximations, consider $\clpred{x\leq 1} \land \clpred{y\geq
    1}$ in a domain with no predicate on~$x-y$.  The operator relaxes
  all upper bounds, yielding~$\clpred{y\geq 1}$ which defines a set
  larger than  the concrete
  time-successors $y\geq 1 \land x-y \leq 0$.
\end{example}

Alternatively, we can also use the method described in~\cite[Theorem
  2]{SB-cav03} to compute time successors, but the above relation will
allow us to compute predecessors as well.


\medskip
Last, we define the reset operation as follows.
For any~$z \in \Clocks$,
\begin{xalignat*}1
  S_{\Reset_z} ={} &\phantom{{}\et{}}
  \bigwedge_{(0,\leq) \leq (k,\mathord{\prec}) \in \Dom_{z,0}}{\clprpr{z-0\prec k}}\\
  &{} \et \bigwedge_{\substack{x \neq z\\(k,\prec) \in \Dom_{x,z}}}
  \Bigl( \bigvee_{\substack{(l,\prec') \in \Dom_{x,0} \\ (l,\prec') \leq (k,\prec) }}
  \clpred{x-0\prec' l} \Bigr)
  \Rightarrow \clprpr{x-z\prec k}
    \\
  &{}\et
  \bigwedge_{\substack{y \neq z  \\ (k,\prec) \in \Dom_{z,y}}}
  \Bigl( \bigvee_{\substack{(l,\prec') \in \Dom_{0,y}\\ (l,\prec') \leq (k,\prec)}}\clpred{0 - y \prec' l} \Bigr)
  \Rightarrow \clprpr{z-y\prec k}\\
  &{}\et
  \bigwedge_{\substack{y \neq z \\(0,\leq) \leq (k,\prec) \in \Dom_{z,y}}} \clprpr{z-y\prec k}\\
  &{}\et
    \bigwedge_{\substack{x, y \neq z \\ (k,\prec) \in \Dom_{x,y}}}
    \clprpr{x-y\prec k} \Leftrightarrow p_{x-y\prec k}.
  \end{xalignat*}
Intuitively, the first conjunct ensures all non-negative upper bounds
on the reset clock hold; the~second conjunct ensures that a diagonal
predicate $x-z\prec k$ with~$x \neq z$ is set to true if, and only if,
an upper bound~$(l,\prec') \leq (k,\prec)$ already holds on~$x$.
Recall that in operations on~DBMs, one~sets such a diagonal component
to the tightest upper bound on~$x$.  The~third conjunct is symmetric
to the second, and the last one ensures diagonals not affected by
reset are unchanged.
Let us define~$\Reset_z(A) = \reduce(\postop_{S_{\Reset_z}}(A))$.

\begin{figure}[t]
  \centering
  \begin{tikzpicture}
    \begin{scope}[scale=.45]
      \fill[black!40] (0,1) -- (2,3) -- (0,3) -- cycle;
      \draw[-latex',line width=.6pt] (0,0) -- (5.5,0);
      \draw[-latex',line width=.6pt] (0,0) -- (0,4.5);
      \node at (0,5) {$y$};
      \node at (6,0) {$x$};
      \begin{scope}[line width=0.1pt]
        \draw[-] (1,0) -- (1,4.5);
        \draw[-] (2,0) -- (2,4.5);
        \draw[-] (3,0) -- (3,4.5);
        \draw[-] (4,0) -- (4,4.5);
        \draw[-] (5,0) -- (5,4.5);
        \draw[-] (0,1) -- (5.5,1);
        \draw[-] (0,2) -- (5.5,2);
        \draw[-] (0,3) -- (5.5,3);
        \draw[-] (0,4) -- (5.5,4);
        \draw[-] (0,0) -- (4.5,4.5);
        \draw[-] (1,0) -- (5.5,4.5);
        \draw[-] (2,0) -- (5.5,3.5);
        \draw[-] (3,0) -- (5.5,2.5);
        \draw[-] (0,1) -- (3.5,4.5);
        \draw[-] (0,2) -- (2.5,4.5);
        \draw[-] (0,3) -- (1.5,4.5);
      \end{scope}
      \begin{scope}[line width=1.5pt,color=red]
        \draw[-] (0,1) -- (3.5,4.5);
        \draw[-] (0,3) -- (5.5,3);
        \draw[-] (4,0) -- (4,4.5);
        \draw[-] (0,1) -- (5.5,1);
        \draw[-] (2,0) -- (5.5,3.5);
      \end{scope}
    \end{scope}
%
    \begin{scope}[scale=.45,shift={(10,0)}]
%      \draw[black!40,line width=4pt] (0,0) -- (4,0);
     \fill[pattern=north west lines, pattern color=blue] (0,0) -- (4,0) -- (4,1) -- (0,1) -- cycle;
     \draw[-latex',line width=.6pt] (0,0) -- (5.5,0);
      \draw[-latex',line width=.6pt] (0,0) -- (0,4.5);
      \node at (0,5) {$y$};
      \node at (6,0) {$x$};
      \begin{scope}[line width=0.1pt]
        \draw[-] (1,0) -- (1,4.5);
        \draw[-] (2,0) -- (2,4.5);
        \draw[-] (3,0) -- (3,4.5);
        \draw[-] (4,0) -- (4,4.5);
        \draw[-] (5,0) -- (5,4.5);
        \draw[-] (0,1) -- (5.5,1);
        \draw[-] (0,2) -- (5.5,2);
        \draw[-] (0,3) -- (5.5,3);
        \draw[-] (0,4) -- (5.5,4);
        \draw[-] (0,0) -- (4.5,4.5);
        \draw[-] (1,0) -- (5.5,4.5);
        \draw[-] (2,0) -- (5.5,3.5);
        \draw[-] (3,0) -- (5.5,2.5);
        \draw[-] (0,1) -- (3.5,4.5);
        \draw[-] (0,2) -- (2.5,4.5);
        \draw[-] (0,3) -- (1.5,4.5);
      \end{scope}
      \begin{scope}[line width=1.5pt,color=red]
        \draw[-] (0,1) -- (3.5,4.5);
        \draw[-] (2,0) -- (5.5,3.5);
        \draw[-] (0,3) -- (5.5,3);
        \draw[-] (4,0) -- (4,4.5);
        \draw[-] (0,1) -- (5.5,1);
      \end{scope}
    \end{scope}

  \end{tikzpicture}
%
  \caption{Reset Operation: The abstract successor of the gray zone on the left is the blue dashed zone on the right.}
  \label{fig:reset}
\end{figure}


%\begin{lemma}
%% \begin{restatable}{lemma}{lemmaopreset}
%% \label{lemma:op-reset}
%%   For any Boolean formula~$A(\Bits,\Pred)$, and~$z\in \Clocks$, we
%%   have $\alpha_\Dom(\zReset_z(\sem{A}_\Dom)) \subseteq \Reset_z(A)$.
%%   Moreover, if~$\Dom$ is the concrete domain, and~$A$ is reduced, then
%%   the above holds with equality.
%% \end{restatable}
%\end{lemma}
\lemmaopreset*

\begin{proof}%[of Lemma~\ref{lemma:op-reset}]
  Let $r = \{z\}$.  We show the equivalent inclusion
  $\zReset_r(\sem{A}_\Dom) \subseteq \sem{\Reset_r(A)}_\Dom$.
  Let~$\nu' \in \zReset_r(\sem{A})$, and $\nu \in \sem{A}$ such
  that~$\nu' = \nu[r\leftarrow 0]$.  So~$u = \alpha_\Dom(\nu) \in
  A$. Letting~$v = \alpha_\Dom(\nu')$, let us show that~$(u,v) \in
  S_{\Reset_r}$, which proves that~$v \in \Reset_r(A)$, thus~$\nu' \in
  \sem{v}_\Dom \subseteq \sem{\Reset_r(A)}_\Dom$.

  \begin{itemize}
  \item Consider~$x \in r$. Since~$\nu'(x) = 0$, we have that~$v
    \models \clpred{x-y\prec k}$ for all $(k,\prec) \in \Dom_{x,y}$
    with~$(k,\mathord\prec) \geq (0,\mathord\leq)$;
    so $(u,v)$ satisfies the first conjunct.
%
    Fix~$(k,\mathord\prec) \in \Dom_{x,y}$.

  \item Assume~$x \not \in r, y \in r$, so that~$\nu'(x) = \nu(x),
    \nu'(y) = 0$.  If there is~$(l,\mathord{\prec'}) \in \Dom_{x,0}$
    with~$(l,\mathord{\prec'}) \leq (k,\mathord\prec)$, this
    means~$\nu(x) - 0 \prec' l \prec k$ so~$\nu'(x) - \nu'(y) \prec
    k$.  Thus the second conjunct is satisfied.

  \item Assume~$x \in r, y \not \in r$ so that~$\nu'(x) = 0, \nu'(y) =
    \nu(y)$.  If there is~$(l,\mathord{\prec'}) \in \Dom_{0,y}$
    with~$(l,\mathord{\prec'}) \leq (k,\mathord\prec)$, this means~$0
    - \nu(y) \prec' l \prec k$ so~$\nu'(x) - \nu'(y) \prec k$ as~well.
    Thus the third conjunct is satisfied.  We also have trivially
    $\nu'(x) - \nu'(y) \prec k $ for all~$(0,\mathord\leq) \leq
    (k,\mathord\prec)$, which entails the fourth conjunct.

  \item Observe that $\nu$ and~$\nu'$ satisfy the same predicates of
    type~$\clpred{x-y\prec \alpha}$ with~$x,y \not \in r$ since these
    values are not affected by the reset; so the pair~$(u,v)$
    satisfies the last conjunct of~$S_{\Reset_r}$ as well.
  \end{itemize}

  %\smallskip

  Now, if the domain is concrete and~$A$ is reduced, then we have
  $\sem{\Reset_r(A)}_\Dom \subseteq \zReset_r(\sem{A}_\Dom)$. In~fact,
  the operation then corresponds precisely to the reset operation in
  DBMs, see~\cite[Algorithm 10]{BY04}.  On~DBMs, for a
  component~$(x,y)$ with~$x \in r, y \not \in r$, the algorithm
  consists in setting this component to value~$(0,y)$. In~our
  encoding, we~thus set the predicate~$\clprpr{x-y\prec k}$ to true
  whenever $\clpred{0-x\prec' l}$ holds with~$(l,\mathord{\prec'})
  \leq (k,\mathord\prec)$.  The argument is symmetric for $(x,y)$
  with~$x \not \in r$, $y \in r$.
\end{proof}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\iffalse

\lemmareduce*

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}%[of Lemma~\ref{lemma:reduce}]
  It is easy to see that $\sem{\reduce_\Dom^k(S)}_\Dom \subseteq \sem{S}_\Dom$.
  In fact, any minterm of the former is a minterm of~$S$ as well by definition.

  To see the converse, consider~$v \in \minterms(S)$. We show
  that~$\sem{v}_\Dom \subseteq \sem{\reduce_\Dom^k(S)}_\Dom$.
  If~$\sem{v}_\Dom = \emptyset$ then the inclusion holds trivially.
  Otherwise, we must have $v \in \minterms(\reduce_\Dom^k(S))$. In
  fact, we show that all minterms~$v \not \in
  \minterms(\reduce_\Dom^k(S))$ satisfy~$\sem{v} = \emptyset$.
  Consider such a minterm~$v$. There must exist~$x,y \in \Clocksz$ and
  $(k,\prec_k) \in \Dom_{x,y}$ such that~$\lnot \clpred{x-y\prec k}$ but
  the right hand side of the implication holds.  But this implies
  that~$\sem{v} = \emptyset$.

  The fact that all miterms of $\reduce_\Dom^k(S)$ are $k$-reduced
  follow by the definition of the operator.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\lemmaemptyrefine*

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}%[of Lemma~\ref{lemma:empty-refine}]
  Consider a (non-canonial) DBM~$D$ that encodes~$v$. Formally, for
  all~$(x,y) \in \Clocksz^2$, $D(x,y) = \min \{ (k,\mathord\prec)
  \mid \clpred{x - y \prec k} \in \Pred_{x,y}\text{ and } v(\clpred{x - y \prec
    k}) = 1\}$.  The~corresponding graph must have a negative
  cycle~$s_1s_2\ldots s_m$ with $s_m = s_1$.  To~define~$\Dom'$,
  we~add the following predicates to~$\Dom$:
  \begin{itemize}
    \item $s_i - s_{i+1} \leq D(s_i,s_{i+1})$ for all~$1\leq j \leq m-1$.
    \item $s_1 - s_{j} \leq D(s_1,s_2) + D(s_2,s_3) + \ldots + D(s_{j-1},s_{j})$
      for~$1\leq j\leq m-1$.
    \end{itemize}
    Intuitively, along the negative cycle, we are adding predicates to
    represent exactly each single step, and also each big step from
    $s_1$ to~$s_j$. This allows to derive the negative cycle using
    only paths of length~$2$.

    More precisely, $v \land \reduce^2_{\Dom'}$ implies the following
    two predicates: $s_1 - s_m \leq \sum_{j=1}^{m-1} D(s_j,s_{j+1})$,
    and $s_m - s_1 \leq D(s_m,s_1)$ as implied by~$v$.  Since
    $-D(s_m,s_1) > \sum_{j=1}^{m-1} D(s_j,s_{j+1})$ due to the
    negative cycle, the~first predicate implies $\lnot \clpred{s_1 -
      s_m \leq -D(s_m,s_1)}$, which contradicts the second one. Hence~$v
    \not \models \reduce^2_{\Dom'}$.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\lemmainter*


\begin{proof}%[of Lemma~\ref{lemma:inter}]
  Consider~$v \in \minterms(A(\Pred) \land B(\Pred))$.  Then $v \in
  \minterms(A(\Pred)) \cap \minterms(B(\Pred))$.  So~$\sem{v}
  \subseteq \sem{A(\Pred)} \cap \sem{B(\Pred)}$, and~$v =
  \alpha_\Dom(\sem{v}) \subseteq \alpha_\Dom(\sem{A(\Pred)}_\Dom \cap
  \sem{B(\Pred)}_\Dom)$.

  We will now show $\alpha_\Dom(\sem{A(\Pred)}_\Dom \cap
  \sem{B(\Pred)}_\Dom) \subseteq A(\Pred) \land B(\Pred)$, which is
  equivalent to $\sem{A(\Pred)}_\Dom \cap \sem{B(\Pred)}_\Dom
  \subseteq \sem{A(\Pred) \land B(\Pred)}$.  Consider any clock
  valuation~$\nu$ in the LHS, and let~$v = \alpha_\Dom(\nu)$.
  Since~$\nu \in \sem{A(\Pred)}_\Dom$ and~$\nu \in
  \sem{B(\Pred)}_\Dom$, we must have $v \in A(\Pred) \land B(\Pred)$,
  so $\nu \in \sem{A(\Pred) \land B(\Pred)}$.
%  By Lemma~\ref{lemma:reduce}, the latter set is equal to~$\sem{A(\Pred) \land B(\Pred)}$.
\end{proof}



\lemmaup*


\begin{proof}%[of Lemma~\ref{lemma:up}]
  We show that 
  $\alpha_\Dom(\timesucc{\sem{A}})\subseteq \Up(A)$,
  which is equivalent to 
  $\timesucc{\sem{A}}\subseteq \sem{\Up(A)}_\Dom$.
  Let~$\nu' \in \timesucc{\sem{A}}$, and let~$\nu \in \sem{A}$ such that
  $\nu' = \nu + d$ for some~$d\geq 0$.
  We write~$u = \alpha_\Dom(\nu)\in \minterms(A)$, and~$v = \alpha_\Dom(\nu')$.
  We now show that~$(u,v) \in S_\Up$. This suffices to prove the inclusion since
  $v \in \minterms(\Up(A))$ implies that~$\nu' \in \sem{v}_\Dom \subseteq \sem{\Up(A)}_\Dom$.
  Observe that $\alpha_\Dom(\nu)$ and~$\alpha_\Dom(\nu')$ satisfy the same diagonal predicates
  of the form~$p_{x-y\prec \alpha}$ with~$x,y \neq 0$, since~$\nu' = \nu+d$.
  Moreover, any lower bound satisfied by~$u$ is also satified by~$v$. Thus, $(u,v) \in S_\Up$.

  \smallskip
  Assume now that~$A$ is reduced. We show that $\Up(A) \subseteq \alpha_\Dom(\timesucc{\sem{A}})$.
  Let~$v \in \minterms(\Up(A))$, and let~$(u,v) \in S_\Up$ with~$u \in \minterms(A)$.
  We claim that~$\sem{v} \subseteq \timesucc{\sem{u}}$.
  This suffices to prove the inclusion since 
  $\{v\} = \alpha_\Dom(\sem{v}) \subseteq \alpha_\Dom(\timesucc{\sem{u}}) \subseteq \alpha_\Dom(\timesucc{\sem{A}})$.
  To~prove the claim, it~suffices to see~$\sem{u}$ and~$\sem{v}$ as DBMs. In fact, $S_\Up$ precisely corresponds to the up operation
  on DBMs. In particular, $u$ and~$v$ have the same diagonal constraints, and any lower bound of~$u$ is a lower bound of~$v$.
  Because~$u$ is reduced, this implies that~$\timesucc{\sem{v}}
  \subseteq \sem{u}$.
\end{proof}


\lemmaopreset*

\begin{proof}%[of Lemma~\ref{lemma:op-reset}]
  Let $r = \{z\}$.  We show the equivalent inclusion
  $\zReset_r(\sem{A}_\Dom) \subseteq \sem{\Reset_r(A)}_\Dom$.
  Let~$\nu' \in \zReset_r(\sem{A})$, and $\nu \in \sem{A}$ such
  that~$\nu' = \nu[r\leftarrow 0]$.  So~$u = \alpha_\Dom(\nu) \in
  A$. Letting~$v = \alpha_\Dom(\nu')$, let us show that~$(u,v) \in
  S_{\Reset_r}$, which proves that~$v \in \Reset_r(A)$, thus~$\nu' \in
  \sem{v}_\Dom \subseteq \sem{\Reset_r(A)}_\Dom$.

  \begin{itemize}
  \item Consider~$x \in r$. Since~$\nu'(x) = 0$, we have that~$v
    \models \clpred{x-y\prec k}$ for all $(k,\prec) \in \Dom_{x,y}$
    with~$(k,\mathord\prec) \geq (0,\mathord\leq)$;
    so $(u,v)$ satisfies the first conjunct.
%
    Fix~$(k,\mathord\prec) \in \Dom_{x,y}$.

  \item Assume~$x \not \in r, y \in r$, so that~$\nu'(x) = \nu(x),
    \nu'(y) = 0$.  If there is~$(l,\mathord{\prec'}) \in \Dom_{x,0}$
    with~$(l,\mathord{\prec'}) \leq (k,\mathord\prec)$, this
    means~$\nu(x) - 0 \prec' l \prec k$ so~$\nu'(x) - \nu'(y) \prec
    k$.  Thus the second conjunct is satisfied.

  \item Assume~$x \in r, y \not \in r$ so that~$\nu'(x) = 0, \nu'(y) =
    \nu(y)$.  If there is~$(l,\mathord{\prec'}) \in \Dom_{0,y}$
    with~$(l,\mathord{\prec'}) \leq (k,\mathord\prec)$, this means~$0
    - \nu(y) \prec' l \prec k$ so~$\nu'(x) - \nu'(y) \prec k$ as~well.
    Thus the third conjunct is satisfied.  We also have trivially
    $\nu'(x) - \nu'(y) \prec k $ for all~$(0,\mathord\leq) \leq
    (k,\mathord\prec)$, which entails the fourth conjunct.

  \item Observe that $\nu$ and~$\nu'$ satisfy the same predicates of
    type~$\clpred{x-y\prec \alpha}$ with~$x,y \not \in r$ since these
    values are not affected by the reset; so the pair~$(u,v)$
    satisfies the last conjunct of~$S_{\Reset_r}$ as well.
  \end{itemize}

  %\smallskip

  Now, if the domain is concrete and~$A$ is reduced, then we have
  $\sem{\Reset_r(A)}_\Dom \subseteq \zReset_r(\sem{A}_\Dom)$. In~fact,
  the operation then corresponds precisely to the reset operation in
  DBMs, see~\cite[Algorithm 10]{BY04}.  On~DBMs, for a
  component~$(x,y)$ with~$x \in r, y \not \in r$, the algorithm
  consists in setting this component to value~$(0,y)$. In~our
  encoding, we~thus set the predicate~$\clprpr{x-y\prec k}$ to true
  whenever $\clpred{0-x\prec' l}$ holds with~$(l,\mathord{\prec'})
  \leq (k,\mathord\prec)$.  The argument is symmetric for $(x,y)$
  with~$x \not \in r$, $y \in r$.
\end{proof}

\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Abstraction refinement}


\lemmarefineup*

\begin{proof}%[of~Lemma~\ref{lemma:refine-up}]
%
  Assume there is~$v \in \timesucc{\sem{A_{1}}} \cap
  \timepred{\sem{A_{2}}}$. There exists~$d_1,d_2\geq 0$ and~$v_1 \in
  A_1$ such that $v = v_1 + d_1$ and~$v+d_2\in A_2$, which
  means~$v_1+d_1+d_2 \in A_2$, thus $\sem{A_1}{\uparrow} \cap
  \sem{A_2}\neq \emptyset$.

  Let~$Z = \sem{\interp(\timesucc{\sem{A_{1}}}, \timepred{\sem{A_{2}}})}$.
  By definition, $\timesucc{\sem{A_1}} \subseteq Z$, and~$Z \cap \timepred{\sem{A_2}} = \emptyset$.
  We have~$\timesucc{Z} = Z$; in~fact, $Z$~cannot have upper bounds since
  $\timesucc{\sem{A_1}}$ does not have~any.
  It~follows that~$\timesucc{Z} \cap \timepred{\sem{A_2}} = \emptyset$.

  Now, consider~$(A_1',A_2') \in \Up^{\alpha'}$ with~$\sem{A_1'}
  \subseteq \sem{A_1}$.
%  Since~$\alpha'$ is obtained by refinement of~$\alpha$, we have 
%  $\sem{A_2'} \subseteq \sem{A_2}$.
  Let us show that~$\sem{A_2'} \subseteq Z$.  Notice that all
  constraints of~$Z$ must be satisfied by~$A_2'$ due to the inclusion
  $\sem{A_1'} \subseteq Z$: there are no upper bounds in~$Z$, all its
  lower bounds are satisfied by~$A_1$, thus also by~$A_1'$, and are
  preserved by definition by~$\Up$, and all diagonal constraints
  of~$Z$ hold in~$A_1$, thus also in~$A_1'$, and are preserved as well
  in~$A_2'$.  This shows the required inclusion.  It~follows
  that~$\sem{A_2'} \cap \sem{A_2} = \emptyset$.
\end{proof}



\lemmarefinereset*

\begin{proof}%[of Lemma~\ref{lemma:refine-reset}]
  Let $v \in \Free_x(\sem{A_{1}}) \cap \Free_x(\sem{A_{2}})$. Then
  there exist~$v_1 \in \sem{A_1}$, $v_2 \in \sem{A_2}$
  and~$v_0$ such
  that~$v_0 = v[x\leftarrow 0] = v_1[x\leftarrow 0] = v_2[x\leftarrow 0]$.
  %such that $v[x\leftarrow 0] = v_1 = v_2$.
  But~$\sem{A_2}$ is
  closed by resetting~$x$, that is, $\sem{A_2}[x:=0] \subseteq
  \sem{A_2}$.  This follows from Lemma~\ref{lemma:op-reset} applied
  to~$A_2$, by~observing that~$A_2$ is unchanged by the reset
  operation.  So~$v_0 \in \sem{A_2}$. But then~$\sem{A_1}[x:=0] \cap
  \sem{A_2} \neq \emptyset$ as witnessed by~$v_1[x:=0] = v_0$.
  %Buth then $v_1(x)=0$, so that $v_1[x\leftarrow 0]=v_2$, witnessing that
  %$\sem{A_1}[x\leftarrow 0] \cap \sem{A_2} \neq \emptyset$.
  
%  Let us write $Z_1 = \Free_x(\sem{A_{1}}$, $Z_2 = \Free_x(\sem{A_{2}})$, and
  Let $Z = \sem{\interp(\Free_x(\sem{A_1}),\Free_x(\sem{A_2}))}$.  For
  all~$A_1'$ satisfying~$\sem{A_1'} \subseteq \sem{A_1}$, we
  have %\todo{why?}~
  $\sem{A_1'}[x \leftarrow 0] \subseteq \sem{A_1}[x\leftarrow 0] \subseteq \Free_x(\sem{A_1}) \subseteq
  Z$. So~$Z \cap A_2 =\emptyset$ means that ${\sem{A_1'}[x\leftarrow 0] \cap
    A_2} = \emptyset$.
\end{proof}



